Two hidden layer suffice: the caterpillar net

Every continuous piecewise linear (CPWL) function is a finite signed sum of maxima of affine functions, making maximum representation a central problem in the study of the expressiveness of ReLU networks. A now-disproved conjecture predicted logarithmic depth for maxima. Inspired by the proof by Brunck et al. (2026) that two hidden layers suffice for general CPWL functions, we give the Caterpillar Net, a nonrecursive construction for the maximum of $N$ inputs with two hidden layers of widths $O(N^2)$ and $2^{O(N\log N)}$. The construction has a direct geometric interpretation.

==> lean-links.tex <==
% Generated by scripts/paper_links.py; do not edit.
\makeatletter
\newcommand{\DeclareSourceEquation}[2]{\expandafter\def\csname paper@lean@#1\endcsname{#2}}
\makeatother
\newcommand{\leanbase}{https://github.com/JayPiZimmermann/Max\_Caterpillar/blob/main}
\DeclareLeanEquation{eq:width}{MaxCaterpillar/Theorems.lean}{18}
\DeclareLeanEquation{eq:count}{MaxCaterpillar/Definitions.lean}{51}
\DeclareLeanEquation{eq:word}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Formula.lean}{130}
\DeclareLeanEquation{eq:faces}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Keys.lean}{29}
\DeclareLeanEquation{eq:face-description}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Keys.lean}{29}
\DeclareLeanEquation{eq:coefficients}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Canonical/Coefficients.lean}{49}
\DeclareLeanEquation{eq:dictionary-span}{MaxCaterpillar/Lemmas.lean}{54}
\DeclareLeanEquation{eq:class-identity}{MaxCaterpillar/Lemmas.lean}{48}
\DeclareLeanEquation{stp:class}{MaxCaterpillar/Lemmas.lean}{48}
\DeclareLeanEquation{eq:geometric-class}{MaxNN/Constructions/Paramid/Geom/Faces/ConeOnly.lean}{71}
\DeclareLeanEquation{stp:corrections}{MaxNN/Constructions/Paramid/Geom/Faces/ConeOnly.lean}{71}
\DeclareLeanEquation{eq:coordinate-deletion}{MaxCaterpillar/Lemmas.lean}{41}
\DeclareLeanEquation{eq:insertion-weight-germs}{MaxNN/Constructions/Paramid/Caterpillar/Coordinate/Structured.lean}{67}
\DeclareLeanEquation{eq:graph}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Spine/GraphKey.lean}{214}
\DeclareLeanEquation{eq:cone-count}{MaxCaterpillar/Lemmas.lean}{66}
\DeclareLeanEquation{eq:features}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/CompactFeatures.lean}{63}
\DeclareLeanEquation{eq:canonical-expansion}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Canonical/Coefficients.lean}{72}
\DeclareLeanEquation{eq:compilation-widths}{MaxCaterpillar/Lemmas.lean}{72}
\DeclareLeanEquation{stp:size-network}{MaxCaterpillar/Lemmas.lean}{72}
\DeclareLeanEquation{eq:asymptotics}{MaxCaterpillar/Theorems.lean}{28}
\DeclareLeanEquation{eq:network-parameters}{MaxCaterpillar/Definitions.lean}{26}
\DeclareLeanEquation{eq:network-evaluation}{MaxCaterpillar/Definitions.lean}{35}
\DeclareLeanEquation{eq:maximum}{MaxCaterpillar/Definitions.lean}{42}
\DeclareLeanEquation{eq:signed-word-sum}{MaxNN/Constructions/Paramid/Caterpillar/Formula/Values.lean}{31}
\DeclareSourceEquation{eq:hinging-maps}{https://doi.org/10.1109/TIT.2005.859246}
\DeclareSourceEquation{eq:hinging-representation}{https://doi.org/10.1109/TIT.2005.859246}
\DeclareLeanEquation{eq:max-hinge}{MaxNN/Core/Relu.lean}{24}
\DeclareLeanEquation{eq:caterpillar-data}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Formula.lean}{24}
\DeclareLeanEquation{eq:word-parent}{MaxNN/Constructions/Paramid/Caterpillar/Words.lean}{28}
\DeclareLeanEquation{eq:word-gamma}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Formula.lean}{122}
\DeclareLeanEquation{eq:edge-functions}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Formula.lean}{126}
\DeclareLeanEquation{eq:edge-comparison}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Formula.lean}{126}
\DeclareLeanEquation{eq:aux_functions}{MaxNN/Constructions/MaxN/Width/Layer/Features.lean}{75}
\DeclareLeanEquation{eq:bases}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Canonical/Average.lean}{26}
\DeclareLeanEquation{eq:gram-matrix}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Canonical/Gram.lean}{147}
\DeclareLeanEquation{eq:gram-rhs}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Canonical/Gram.lean}{201}
\DeclareLeanEquation{eq:inner-product}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Canonical/Gram.lean}{50}
\DeclareLeanEquation{eq:basis-expansion}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Canonical/Average.lean}{61}
\DeclareLeanEquation{eq:normal-equations}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Canonical/Gram.lean}{220}
\DeclareLeanEquation{eq:average-expansion}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Canonical/Coefficients.lean}{53}
\DeclareLeanEquation{eq:hinge-reversal}{MaxNN/Core/Relu.lean}{33}
\DeclareLeanEquation{eq:remainder}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/AbsorbHinges.lean}{95}
\DeclareLeanEquation{eq:remainder-translation}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/CompactCovariance.lean}{74}
\DeclareLeanEquation{eq:simplex}{MaxNN/Constructions/Paramid/Geom/Defs.lean}{121}
\DeclareLeanEquation{eq:support-function}{MaxNN/Constructions/Paramid/Geom/Defs.lean}{43}
\DeclareLeanEquation{eq:unit-polytope}{MaxNN/Constructions/Paramid/Geom/Boundary/ConeFaces.lean}{400}
\DeclareLeanEquation{eq:face-normal}{MaxNN/Constructions/Paramid/Geom/Defs.lean}{62}
\DeclareLeanEquation{eq:exposed-face}{MaxNN/Constructions/Paramid/Geom/Defs.lean}{62}
\DeclareLeanEquation{eq:facet-difference}{MaxNN/Constructions/Paramid/Geom/Germ.lean}{460}
\DeclareLeanEquation{eq:face-derivative}{MaxNN/Constructions/Paramid/Geom/Germ.lean}{364}
\DeclareLeanEquation{eq:facet-error}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Formula.lean}{184}
\DeclareLeanEquation{eq:linear-facet}{MaxNN/Constructions/Paramid/Caterpillar/Formula/Braid.lean}{96}
\DeclareLeanEquation{eq:lifted-induction}{MaxNN/Constructions/Paramid/Caterpillar/Formula/Lift.lean}{40}
\DeclareLeanEquation{eq:induction-error-split}{MaxNN/Constructions/Paramid/Caterpillar/Formula/Assembly.lean}{69}
\DeclareLeanEquation{eq:root-star}{MaxNN/Constructions/Paramid/Caterpillar/Coordinate/Star.lean}{25}
\DeclareLeanEquation{eq:boolean-cancellation}{MaxNN/Constructions/Paramid/Caterpillar/Words/RootStar.lean}{47}
\DeclareLeanEquation{eq:full-coordinates}{MaxNN/Constructions/Paramid/Geom/Coordinates.lean}{27}
\DeclareLeanEquation{eq:head-count-bound}{MaxCaterpillar/Asymptotics.lean}{31}
\DeclareLeanEquation{eq:cone-growth}{MaxCaterpillar/Asymptotics.lean}{44}
\DeclareLeanEquation{eq:second-growth}{MaxCaterpillar/Asymptotics.lean}{54}
\DeclareLeanEquation{eq:first-growth}{MaxCaterpillar/Asymptotics.lean}{17}
\DeclareLeanEquation{eq:absorbed-pairs}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/AbsorbHinges.lean}{26}
\DeclareLeanEquation{eq:recover-coordinates}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/CompactFeatures.lean}{111}
\DeclareLeanEquation{eq:feature-count}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/CompactFeatures.lean}{21}
\DeclareLeanEquation{eq:normalized-description}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Normalize.lean}{24}
\DeclareLeanEquation{eq:facet-reduction}{MaxCaterpillar/Lemmas.lean}{33}
\DeclareLeanEquation{stp:reconstruction}{MaxCaterpillar/Lemmas.lean}{33}
\DeclareLeanEquation{eq:base-unit}{MaxNN/Constructions/Paramid/Caterpillar/Coordinate/Base.lean}{78}
\DeclareLeanEquation{eq:base-formula}{MaxNN/Constructions/Paramid/Caterpillar/Coordinate/Base.lean}{84}
\DeclareLeanEquation{eq:simplex-facet}{MaxNN/Constructions/Paramid/Caterpillar/Formula/SimplexGerms.lean}{60}
\DeclareLeanEquation{eq:kuhn-simplices}{MaxNN/Constructions/Paramid/Geom/Kuhn.lean}{43}
\DeclareLeanEquation{eq:kuhn-support-error}{MaxNN/Constructions/Paramid/Geom/Kuhn.lean}{320}
\DeclareLeanEquation{eq:apex-maximum}{MaxNN/Constructions/Paramid/Caterpillar/Geometry/Paramid.lean}{43}
\DeclareLeanEquation{eq:retained-count}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/HingeCount.lean}{166}
\DeclareLeanEquation{stp:size-count}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/HingeCount.lean}{166}
\DeclareLeanEquation{eq:face-dimension-drop}{MaxNN/Constructions/Paramid/Geom/Flag.lean}{200}
\DeclareLeanEquation{eq:error-peeling}{MaxNN/Constructions/Paramid/Geom/Faces/Peel.lean}{38}
\DeclareLeanEquation{eq:simplex-vertex-removal}{MaxNN/Constructions/Paramid/Geom/Faces/ConeOnly/SimplexGerm.lean}{184}
\DeclareLeanEquation{eq:initial-simplex-error}{MaxNN/Constructions/Paramid/Geom/Faces/ConeOnly/LocalIdentity.lean}{205}
\DeclareLeanEquation{eq:simplex-deletion-sign}{MaxNN/Constructions/Paramid/Geom/Faces/ConeOnly/SimplexGerm.lean}{195}
\DeclareLeanEquation{eq:simplex-induction-use}{MaxNN/Constructions/Paramid/Geom/Faces/ConeOnly.lean}{40}
\DeclareLeanEquation{eq:residual-invariant}{MaxNN/Constructions/Paramid/Geom/Faces.lean}{69}
\DeclareLeanEquation{eq:support-cut}{MaxNN/Constructions/Paramid/Geom/Sweep/Support.lean}{142}
\DeclareLeanEquation{eq:sweep-support-high}{MaxNN/Constructions/Paramid/Geom/Sweep.lean}{187}
\DeclareLeanEquation{eq:sweep-support-translate}{MaxNN/Constructions/Paramid/Geom/Sweep.lean}{304}
\DeclareLeanEquation{eq:sweep-operation}{MaxNN/Constructions/Paramid/Geom/Defs.lean}{106}
\DeclareLeanEquation{eq:sweep-dimension}{MaxNN/Constructions/Paramid/Geom/Sweep.lean}{366}
\DeclareLeanEquation{eq:simplex-reconstruction}{MaxNN/Constructions/Paramid/Geom/Reconstruct.lean}{83}
\DeclareLeanEquation{eq:simplex-isolate-facet}{MaxNN/Constructions/Paramid/Geom/Reconstruct/FacetGerm.lean}{268}
\DeclareLeanEquation{eq:normalized-facet-normal}{MaxNN/Constructions/Paramid/Geom/Reconstruct/FacetGerm.lean}{185}
\DeclareLeanEquation{eq:facet-group-bound}{MaxNN/Constructions/Paramid/Geom/Reconstruct/FacetGerm.lean}{326}
\DeclareLeanEquation{eq:single-facet-group}{MaxNN/Constructions/Paramid/Geom/Reconstruct/FacetGerm.lean}{326}
\DeclareLeanEquation{eq:translation-invariance}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/CompactCanonical.lean}{22}
\DeclareLeanEquation{eq:tag-family}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Canonical/Table.lean}{93}
\DeclareLeanEquation{eq:tagged-coefficients}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Canonical/Coefficients.lean}{93}
\DeclareLeanEquation{eq:tagged-expansion}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Canonical/Coefficients.lean}{110}
\DeclareLeanEquation{eq:normalized-tag-coefficients}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Canonical/Table.lean}{166}
\DeclareLeanEquation{eq:active-normalized-descriptions}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/Canonical/Table.lean}{171}
\DeclareLeanEquation{eq:retained-descriptions}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/AbsorbHinges.lean}{31}
\DeclareLeanEquation{eq:ridge-cut-residual}{MaxNN/Constructions/Paramid/Geom/Reconstruct/SimplexCut.lean}{613}
\DeclareLeanEquation{eq:simplex-support-expansion}{MaxNN/Constructions/Paramid/Caterpillar/Formula/Completeness.lean}{80}
\DeclareLeanEquation{eq:direction-pattern}{MaxNN/Constructions/Paramid/Caterpillar/Geometry/Facets/Pattern.lean}{64}
\DeclareLeanEquation{eq:braid-reflection}{MaxNN/Constructions/Paramid/Caterpillar/Formula/Braid.lean}{66}
\DeclareLeanEquation{eq:braid-germ}{MaxNN/Constructions/Paramid/Geom/Germ/Reflection.lean}{34}
\DeclareLeanEquation{eq:block-pairing}{MaxNN/Constructions/Paramid/Caterpillar/Geometry/Toggle.lean}{42}
\DeclareLeanEquation{eq:lower-arity-translation}{MaxNN/Constructions/Paramid/Caterpillar/Formula/Lift.lean}{30}
\DeclareLeanEquation{eq:coordinate-active}{MaxNN/Constructions/Paramid/Caterpillar/Coordinate/Active.lean}{20}
\DeclareLeanEquation{eq:coordinate-fibre-partition}{MaxNN/Constructions/Paramid/Caterpillar/Coordinate/ReindexActive.lean}{228}
\DeclareLeanEquation{eq:root-star-average}{MaxNN/Constructions/Paramid/Caterpillar/Coordinate/Star.lean}{315}
\DeclareLeanEquation{eq:lower-caterpillar-summand}{MaxNN/Constructions/Paramid/Caterpillar/Coordinate/Structured.lean}{23}
\DeclareLeanEquation{eq:auxiliary-remainder}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/CompactCovariance.lean}{22}
\DeclareLeanEquation{eq:compact-remainder}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/CompactCovariance.lean}{89}
\DeclareLeanEquation{eq:network-assembly}{MaxCaterpillar/Construction.lean}{39}
\DeclareLeanEquation{eq:signed-remainder}{MaxNN/Constructions/Paramid/Caterpillar/Corrections/CompactCanonical.lean}{57}
\DeclareLeanEquation{eq:coordinate-relabel}{MaxNN/Constructions/Paramid/Caterpillar/Formula/CoordinateDirections.lean}{119}

